SOL: Safe On-Node Learning in Cloud Platforms

Cloud platforms run many software agents on each server node. These agents manage all aspects of node operation, and in some cases frequently collect data and make decisions. Unfortunately, their behavior is typically based on pre-defined static heuristics or offline analysis; they do not leverage on-node machine learning (ML). In this paper, we first characterize the spectrum of node agents in Azure, and identify the classes of agents that are most likely to benefit from on-node ML. We then propose SOL, an extensible framework for designing ML-based agents that are safe and robust to the range of failure conditions that occur in production. SOL provides a simple API to agent developers and manages the scheduling and running of the agent-specific functions they write. We illustrate the use of SOL by implementing three ML-based agents that manage CPU cores, node power, and memory placement. Our experiments show that (1) ML substantially improves our agents, and (2) SOL ensures that agents operate safely under a variety of failure conditions. We conclude that ML-based agents show significant potential and that SOL can help build them.

==> challenges.tex <==
% %!TEX root =asplos22-paper-main.tex
% \section{Challenges of On-node Learning}
% Despite the many advantages learning on the node brings, there are numerous challenges that need to be addressed in order to make it safe and robust. 
% In the typical off-node learning setting, a model is trained offline and then deployed to serve inference. The deployed model shows more predictable accuracy because the training data captures well the characteristics of data observed during inference.  
% In contrast to off-node learning, on-node learning builds models online without a-priori information. Although models learned online are more general and up-to-date, they experience higher performance variability as the environment and their subject of learning undergo constant changes. Below we discuss different factors that can degrade the performance and efficiency of on-node learning agents when they are deployed.
%
% \dan{Include a discussion here about failure detection in ML models can be tricky to detect,
% as the models themselves can produce useless predictions without breaking any code. Garbage In, Garbage Out.}
%
% \subsection{Unpredictable Resource Availability}
% %\subsection{Stale Predictions}
% The top goal of a cloud provider is to offer reliable and performant service to its users. In order to achieve this goal, cloud tenant workloads reserves the highest priority over server nodes resources. The on-node learning agents therefore need to be blocked or throttled during periods of low resource availability to minimize interference with tenant workloads. When this happens, the node agents may experience arbitrarily long scheduling delays. For example, the agent could take an action based on stale prediction that no longer represent the current workload characteristics. The agent could also be stuck in the state from a prior action for too long because it has not been able to produce a new prediction in time. Since most on-node learning agents need to run in tight response loops, such scheduling delays due to resource unavailability can be detrimental to their performance. 
%
% \subsection{Invalid Data Readings}
% Correctness of data is a more crucial in on-node learning because the model is updated online with live data. Frequent invalid data readings can pass wrong information to the model that severely reduce its prediction accuracy. The heterogeneity of server nodes further complicates the problems. Server nodes in the data center run on different software and hardware. These differences can impose challenges depending what data is required by the learning agents. For example, the Intel servers will not have the same set of hardware counters counters as AMD servers. The same learning agent may be deployed to any type of server node, thus it needs to account for server heterogeneity and ensures it collects data from the right sources when deployed. \yawen{not sure if our data validation safeguard is the best place to addresses the heterogeneous sw/hw problem, this seems more like a one-time check \& config in agent initialization.}
% \dan{Notes: Semantics of data can change (units, scale,  etc). In the telemetry collection case, these changes
% can be handled after the fact offline, but in the on-node case they will be immediately consumed and can
% break the model.}
%
% \subsection{Varying Model Accuracy}
% On-node learning agents will show low accuracy when the design of the model is broken or the workloads it tries to predict for are more un-learnable.
% Yet models are simply functions that will always produce a prediction given a valid input, even if the
% contents of the input are garbage or the model has not learned any useful patterns.
% When learning fails, the agent will act based on wrong predictions. These actions likely involve resource adjustment decisions that can negatively impact client workloads. When this goes undetected, the client workloads continuously suffer from poor performance. Client workloads that have stringent performance requirements will be even more sensitive to mis-predictions from the learning agents.    
%
% \subsection{Node Performance and Reliability}
% Deploying on-node learning agents in the public cloud creates the additional challenge of not having access to application-level metrics from client workloads. This is because client workloads are often run inside VMs as opaque-boxes. On-node learning agents do not have a direct way of measuring the performance of client workloads. Instead, the learning agents must estimates their performance impacts on clients workloads from external signals such as vCPU dispatch wait time \cite{wang2021smartharvest}. Sometimes cloud servers run in stressed or constrained modes such as being over-subscribed or power-capped. In such settings, there may be little room for efficiency improvement from on-node learning. Harmful consequences from a bad prediction may also get exacerbated, making learning on the node 
% entirely un-beneficial. 
%
% \subsection{Ad-hoc Implementation}
% Most learning-based resource management agents from recent works use ad-hoc implementations that are management task-specific. These ad-hoc implementations limit the applicability of the designs and also require high maintenance efforts. 

